Replicating Persistent Memory Key-Value Stores with Efficient RDMA Abstraction

Combining persistent memory (PM) with RDMA is a promising approach to performant replicated distributed key-value stores (KVSs). However, existing replication approaches do not work well when applied to PM KVSs: 1) Using RPC induces software queueing and execution at backups, increasing request latency; 2) Using one-sided RDMA WRITE causes many streams of small PM writes, leading to severe device-level write amplification (DLWA) on PM. In this paper, we propose Rowan, an efficient RDMA abstraction to handle replication writes in PM KVSs; it aggregates concurrent remote writes from different servers, and lands these writes to PM in a sequential (thus low DLWA) and one-sided (thus low latency) manner. We realize Rowan with off-the-shelf RDMA NICs. Further, we build Rowan-KV, a log-structured PM KVS using Rowan for replication. Evaluation shows that under write-intensive workloads, compared with PM KVSs using RPC and RDMA WRITE for replication, Rowan-KV boosts throughput by 1.22X and 1.39X as well as lowers median PUT latency by 1.77X and 2.11X, respectively, while largely eliminating DLWA.

==> secs/background.tex <==
% \section{Background}
% \label{sec:bg}

% \cite{ArtOfMultiprocessor}
